Resource-Constrained Adaptive Search and Tracking for Sparse Dynamic Targets

This paper considers the problem of resource-constrained and noise-limited localization and estimation of dynamic targets that are sparsely distributed over a large area. We generalize an existing framework [Bashan et al, 2008] for adaptive allocation of sensing resources to the dynamic case, accounting for time-varying target behavior such as transitions to neighboring cells and varying amplitudes over a potentially long time horizon. The proposed adaptive sensing policy is driven by minimization of a modified version of the previously introduced ARAP objective function, which is a surrogate function for mean squared error within locations containing targets. We provide theoretical upper bounds on the performance of adaptive sensing policies by analyzing solutions with oracle knowledge of target locations, gaining insight into the effect of target motion and amplitude variation as well as sparsity. Exact minimization of the multi-stage objective function is infeasible, but myopic optimization yields a closed-form solution. We propose a simple non-myopic extension, the Dynamic Adaptive Resource Allocation Policy (D-ARAP), that allocates a fraction of resources for exploring all locations rather than solely exploiting the current belief state. Our numerical studies indicate that D-ARAP has the following advantages: (a) it is more robust than the myopic policy to noise, missing data, and model mismatch; (b) it performs comparably to well-known approximate dynamic programming solutions but at significantly lower computational complexity; and (c) it improves greatly upon non-adaptive uniform resource allocation in terms of estimation error and probability of detection.

==> darap_Introduction6.tex <==
Systems for wide area surveillance such as the Gotcha synthetic aperture radar and the Angel Fire electro-optical sensor currently offer %provide the opportunity for 
near real-time imaging and surveillance of city-sized scenes.  Generally, these systems perform continuous collection of data, followed by forensic analysis to detect and track targets within the scene. The amount of raw data incurred by these systems is often very large, even though the interesting features (e.g. moving targets, etc.) may be sparsely distributed. %located throughout the scene. 
Thus, there is a high likelihood that sensing and/or computational resources may be wasted by searching areas where targets are not located.  Abidi et al \cite{abidi2008survey} provides a comprehensive survey of recent work in wide-area surveillance, including topics in coverage analysis, optimal sensor positioning and sensor fusion.  Moreover, they stress the need for intelligent data analysis and capture systems in order to deal with the large data problem. 

In adaptive sampling, past observations are used %in order 
to inform the collection %sensing/sampling 
of future observations, generally with the goal of focusing effort onto the ``interesting'' regions of the search space. Adaptive sampling can therefore be an important % substantial 
tool for efficiently managing the large data problem faced %incurred 
by wide-area surveillance systems.  Previous work has shown that adaptive sampling can significantly improve performance in localizing a few targets in noisy backgrounds \cite{Castro-04-coarse-to-fine,Castro-05-faster-rate-reg-via-act-learn, Bashan-08-opt-2-stage-search, bashan2011marapTSP, Hitchings_Castanon_AdaptiveSensing2010, haupt2011distilled, haupt2012sequentially, Wei-Hero-multistage-adaptive-estimation-of-sparse-signals,malloy2012sequential,MalloyAdaptiveCompressed13} in comparison to a uniform policy that uses equal sensing effort across the scene.  Benefits include gains in estimation precision \cite{Bashan-08-opt-2-stage-search, bashan2011marapTSP}, provable detection of the targets often at faster convergence rates \cite{haupt2011distilled}, and improved robustness in detection performance as measured by the minimum detectable amplitudes \cite{haupt2012sequentially}.  

Bashan et al \cite{Bashan-08-opt-2-stage-search} provided an optimal two-stage policy called ARAP for adaptively localizing targets and estimating their amplitudes in noise under effort budget constraints.  A  multiscale approach was also introduced in order to reduce the total number of %required 
measurements \cite{bashan2011marapTSP}.  Hitchings and Castanon \cite{Hitchings_Castanon_AdaptiveSensing2010} provided an online modification to \cite{Bashan-08-opt-2-stage-search} through Lagrangian constraint relaxation.  Additionally, \cite{Wei-Hero-multistage-adaptive-estimation-of-sparse-signals} extended the two-stage policy to an arbitrary number of stages using approximate dynamic programming, %solutions, 
and generalized the framework to allow for a variety of measurement/estimation loss models.  Using a similar model, Distilled Sensing \cite{haupt2011distilled,haupt2012sequentially} specified a methodology for locating targets in noise at much lower signal-to-noise ratios (SNR) than non-adaptive methods. Malloy et al \cite{malloy2012sequential} extends Distilled Sensing to non-Gaussian models, while \cite{MalloyAdaptiveCompressed13,haupt2012sequentially} consider compressive measurements.

In the above methods, it is assumed that the targets of interest remain stationary across sensing/observation epochs.  In wide-area surveillance, however, many targets %of the targets of interest will 
exhibit complex dynamic behavior such as movement, entering/leaving the scene, and  obscuration.   Krishnamurthy \cite{Krishnamurthy-01-hmm-mab-beam-sched} considers the problem of selecting where to point an agile sensor in order to track $P$ moving targets among a finite number of cells.  When the state is fully observable, the problem can be posed as a Markov decision process (MDP) with well-known solutions.  Krishnamurthy formulates the problem as a hidden Markov model (HMM) tracking problem in the more practical case where the state is observed with noise. %y measurements.  
He %provides 
discusses an optimal policy which depends on the individual target's belief state - the conditional density of the state given the observation history.  Moreover, a suboptimal approach to estimating the Gittins index is provided to combat the prohibitive computational complexity of the optimal solution.

Chong et al. \cite{chong2008monte} shows that many adaptive sensing problems can be formulated as partially observable Markov decision processes (POMDPs).  This general framework is concerned with selecting actions to maximize the sum of an immediate reward and an expected future reward, given a system with Markovian evolution but only partially observable state (e.g.\ due to noise).  Unfortunately, 
%Informally, a POMDP consists of a state space, an action space, and an observation space (the sets of possible states, actions, and observations, respectively), coupled with a state transition law, an observation law that specifies the distribution of the observations given a belief state $b$ and action $a$, and a reward function $r(b,a)$.  In general, the determination of optimal actions involves both the immediate reward as well as the expected future reward, where the latter 
the expected future reward is often difficult to compute, while the tractability of the optimal solution is further impaired when the state space and action space are large. Chong et al. \cite{chong2008monte} describes in detail approximate methods that include parametric approximations, reinforcement learning techniques, and rollout policies.  The last of these % In particular, rollout policies 
assumes that a base policy is available that may not be optimal but is simple to compute.   Rollout policies then ensure policy improvement, i.e., they are guaranteed to do at least as well as the base policy.  However, rollout policies still remain impractical in cases where the action space is large. 

\ignore{Informally, a POMDP consists of
\begin{itemize}
\item a set of possible states (the state space).
\item a set of possible actions (the action space)
\item a set of possible observations (the observation space)
\item  $r(b_t,a)$, a reward (or cost) function received given an action $a$ taken at a state $b_t$.
\item a state transition law (i.e., distribution)
\item an observation law specifying the distribution of observations given an action taken at a state.
\end{itemize}
Given the current belief state, Bellman's principle states that the optimal objective function value starting from belief state $b_0$ is given by
\begin{equation}
V_T^*(b_0) = \max\limits_a \left( r(b_0,a) + \mathbb{E}[V_{T-1}^*(b_1) | b_0,a]\right).
\end{equation}
Note that $V_T^*(b_0)$ is defined recursively where each subsequent stage chooses the optimal action $a$.  The $Q$-value of an action $a$ at time $t$ with belief state $b_t$ is defined as
\begin{equation}
Q_{T-t}(b_t,a) = r(b_t,a) + \mathbb{E}[V_{T-t-1}^*(b_{t+1}) | b_t,a].
\end{equation}
Bellman's principle can be rewritten as stating the optimal action as being the action that maximizes the $Q$-value:
\begin{equation}
\pi_t^*(b_t) = \arg\max\limits_a Q_{T-t}(b_t,a).
\end{equation}
The $Q$-values are composed of two parts: (a) the immediate reward of taking action $a$, and (b) the expected cumulative reward for the remaining stages assuming optimal actions are taken.  Generally, the first part can be computed in a straightforward manner, but the latter part requires significant and possibly intractable computation.  , particularly when the belief state space and action spaces are large.  Chong et al. \cite{chong2008monte} describes approximate methods in detail that include parametric approximations, reinforcement learning techniques, and rollout policies.   In particular, rollout policies assume that a base policy is available that may not be optimal (as in Bellman's principle), but is simple to compute.  In this case, the $Q$-values can be approximated as 
\begin{equation}
Q^{base}(b,a) = r(b,a) + \mathbb{E}[V^{base}(b')|b,a].
\end{equation}
Computation of the approximate $Q$-values still involves expectations over remaining stages, but removes the degrees of freedom in finding the ``optimal'' actions. } 

%In this paper, we provide a Bayesian formulation akin to \cite{Bashan-08-opt-2-stage-search}, namely the Dynamic Adaptive Resource Allocation Policy (D-ARAP), where the goal is to localize and estimate  moving targets in noise under resource constraints.  This approach can simultaneously account for multiple targets as well as continuous allocation of sensing resources, as opposed to the discrete sensing choices optimized in \cite{Krishnamurthy-01-hmm-mab-beam-sched}.  Moreover, the proposed framework is flexible in terms of %the definition of 
%the dynamic target state model with the requirement that the posterior belief state can be efficiently estimated (e.g. with a Kalman or particle filter).  
In this paper, the lower complexity Bayesian formulation of adaptive sampling introduced in \cite{Bashan-08-opt-2-stage-search} is extended to targets that are dynamic as well as sparse, encompassing target motion, appearance and disappearance, and amplitude variation.  This formulation can simultaneously account for multiple targets as well as continuous allocation of sensing resources, as opposed to the discrete sensing choices optimized in \cite{Krishnamurthy-01-hmm-mab-beam-sched}.  To facilitate resource allocation, we provide an efficient approximation to the target posterior distribution and a multistage extension of the cost function in \cite{Bashan-08-opt-2-stage-search}.  
Based on this framework, we then propose the Dynamic Adaptive Resource Allocation Policy (D-ARAP), a non-myopic policy for adaptive sampling that achieves a favorable trade-off between performance and planning complexity.  Our analysis suggests that as compared to approximate POMDP solutions, in particular rollout policies, D-ARAP performs well but at a fraction of the computational cost.  Compared to myopic policies, D-ARAP has increased robustness to noise, missing data, and model mismatch.  Lastly, compared to the non-adaptive uniform policy, D-ARAP continues to yield large improvements in estimation and detection performance similar to the static case \cite{Bashan-08-opt-2-stage-search,Wei-Hero-multistage-adaptive-estimation-of-sparse-signals}.

For static targets, it is known  \cite{Bashan-08-opt-2-stage-search,Wei-Hero-guarantees-adaptive-estimation-sparse-signals} that estimation gains due to adaptive sampling increase with the sparsity of the targets.  The present work extends understanding of the potential benefits of adaptation to the dynamic setting.  Our aim is to understand the potential benefits of adaptive sensing for targets that are dynamic as well as sparse, thus extending \cite{Bashan-08-opt-2-stage-search, bashan2011marapTSP,Wei-Hero-multistage-adaptive-estimation-of-sparse-signals}. 
By analyzing policies with oracle knowledge of target locations, we derive upper bounds on the performance of realizable policies.  The bounds confirm the dependence on sparsity for dynamic targets and additionally characterize the effect of target motion and amplitude variation on the potential gain.  Moreover, simulations indicate that D-ARAP can approach these oracle bounds as the SNR and number of planning stages increase. 

\ignore{The current paper improves upon our previous work \cite{NewstadtWeiHeroCAMSAP13,NewstadtBashanHeroAsilomar2011} by providing an offline rollout policy in Section \ref{darap-sec:adaptive-policy} whose training complexity scales linearly with the number of stages, with no noticeable performance degradation compared to the nested policy in \cite{NewstadtWeiHeroCAMSAP13} that had quadratic complexity.  In addition, Section \ref{darap-sec:theory} on theoretical performance bounds is new, simulation results have been significantly expanded, and the presentation of our framework has been refined. }

%D-ARAP has several interesting properties in comparison to alternative frameworks for allocating limited resources to localizing moving targets.  First, it has significant performance gains over the baseline policy that uniformly allocates resources across the scene, in terms of estimation error and detection probability.  Second, D-ARAP empirically performs at a similar level to POMDP approximate solutions, in particular rollout policies, albeit at a fraction of the computational cost.  Finally, D-ARAP has increased robustness to noise and model mismatch as compared to myopic policies.

The rest of this paper is organized as follows.  %We provide notation in Section \ref{darap-sec:notation}. 
We formalize the problem in Section \ref{darap-sec:problem-formulation} and present adaptive sensing policies in Section \ref{darap-sec:adaptive-policy}.  We %provide theoretical comparisons to the baseline and oracle policies 
derive performance bounds for adaptive sensing of dynamic targets in Section \ref{darap-sec:theory}. Numerical performance analysis is given in Section \ref{darap-sec:performance-analysis}.  In Section \ref{darap-sec:conclusion}, we conclude and discuss future directions.


==> darap_Notation.tex <==
\begin{itemize}
\item $Q$ - Number of cells in search space.
\item $T$ - Number of stages (time).
\item $t$ - Current time, $t\in 1,2,\dots,T$.
\item ${\cal X}=\{1,2,\ldots,Q\}$ - Discrete space of $Q$ cells.
\item $\Psi(t) \subseteq {\cal X}$ - Subset of $\cal X$, a.k.a. the ROI at time $t$.
\item $I_i(t)$ - indicator function of the ROI such that
\begin{equation}\label{darap-eq:ROI_indic}
I_i(t)=\begin{cases}1,&i\in\Psi(t)\\0,&{\rm
Otherwise}\end{cases} \hspace{0.1in} \mathrm{for}\ i\in\{1,2,\dots,Q\}.
\end{equation}
\item $\widehat \Psi(t)\subseteq {\cal X}$ - Estimated ROI, learned from measurements.
\item $\lambda_i(t) \in [0,\Lambda(t)]$ - Search effort in cell $i$ at stage $t$.
\item $\Lambda(t) = \sum\limits_{i=1}^Q \lambda_i(t)$ - Total search effort at stage $t$.
\item $\vY(t) = \{\vy(1),\vy(2),\dots,\vy(t)\}$ - Measurement history.
\ignore{\item ${p}_{I_j(t)|\vY (t')}$ - Posterior probability at time $t$ for target existence in the $j$-th cell given measurements up until time $t'$.}
\item $\kappa(t)\in[0,1]$ - Percentage of resource budget to be used for exploration of $\cal X$ rather than exploitation of $\hat{\Psi}(t)$.
\end{itemize}

\subsection{For dynamic target state model}
\begin{itemize}
\item $\alpha$ - Target birth probability.
\item $\beta$ - Target death probability.
\item $\pi_0$ - Probability that target remains in cell in consecutive stages.
\item $G(i)\subseteq\calX$ - Set of neighbors of cell $i$.
\item {\color{red} $\tilde{N}(t)$ - Number of targets in scene at stage $t$.}
\item ${\mu}_i(t)$ - Estimate of $\theta_i(t)$ at stage $t$ given $\vY(t-1)$.
\item $\sigma_i^2(t)$ - Variance of $\theta_i(t)$ at stage $t$ given $\vY(t-1)$.
\item $p_i(t) = \Pr(I_i(t)=1|\vY(t-1))$ - Posterior probability of target existence.
\item ${\bf x}(t) = \set{p_i(t), {\mu}_i(t), \sigma_i^2(t)}_{i=1}^Q$ - Belief state at stage $t$.
\end{itemize}

